Non-linear Kalman filters for calibration in radio interferometry

We present a new calibration scheme based on a non-linear version of Kalman filter that aims at estimating the physical terms appearing in the Radio Interferometry Measurement Equation (RIME). We enrich the filter's structure with a tunable data representation model, together with an augmented measurement model for regularization. We show using simulations that it can properly estimate the physical effects appearing in the RIME. We found that this approach is particularly useful in the most extreme cases such as when ionospheric and clock effects are simultaneously present. Combined with the ability to provide prior knowledge on the expected structure of the physical instrumental effects (expected physical state and dynamics), we obtain a fairly cheap algorithm that we believe to be robust, especially in low signal-to-noise regime. Potentially the use of filters and other similar methods can represent an improvement for calibration in radio interferometry, under the condition that the effects corrupting visibilities are understood and analytically stable. Recursive algorithms are particularly well adapted for pre-calibration and sky model estimate in a streaming way. This may be useful for the SKA-type instruments that produce huge amounts of data that have to be calibrated before being averaged.

==> Initialisation.tex <==
\section{Initialization and regularization}
\label{sec:init}

The Kalman Filter is designed to track the process state, but requires
initialization of $\hat{\textbf{x}}_{0\mid 0}$ and
$\textbf{P}_{0\mid0}$. The main difficulty when directly estimating
the underlying physical parameter instead of the effective Jones
matrices, lies in the high non-linearity of some of the process vector
variables. 


\def\MJx{\textbf{J}_{\textbf{x}_i}}
\def\MJd{\textbf{J}^{\#}}
\def\Bdelta{\large\bm{\mathcal{\delta}_{\textbf{x}_i}}}


\subsection{Pseudo-Inverse step to constrain clock offsets}
\label{sec:InitClock}

In the case of interferometers that do not have distributed clocks
(such as LOFAR),
individual clock are attached to each stations or to sub-groups of
stations. 
Solving for the clocks individual offsets make the predicted visibilities
rotate and wrap rapidly along the frequency axis. Intuitively, this
makes the Jacobian very sensitive to small perturbations in the
process domain.

The time errors offsets create frequency dependent phase
errors at the correlation level, and we can write the corrupted
visibility $\text{V}^c_{pq}$ as:

\begin{alignat}{3}
\text{V}^c_{pq}(\nu)&=\text{V}^t_{pq}(\nu)\exp{\left(
2\pi i \nu \Delta t_{pq}
\right)}
\end{alignat}

\noindent where $\text{V}^t_{pq}$ is the true visibility, $\Delta
t_{pq}=\Delta t_{p0}-\Delta t_{q0}$ is the time error between antenna
$p$ and antenna $q$ (taking the $1^{st}$ antenna as the time reference
for example). Taking the power spectrum of the model-normalized
corrupted signal, we can get $\Delta t_{pq}$ for each baseline $(pq)$.

\begin{alignat}{3}
\label{eq:tpq}
\widehat{\Delta t_{pq}}&=\underset{t}{\operatorname{arg\,max}}\left|
\mathcal{F}_t\left(
\frac{\text{V}^c_{pq}}{\text{V}^t_{pq}}
\right)
\right|^2
\end{alignat}

We then write $\bm{\Delta t}$ as a vector of size $n_{\mathrm{a}}$ (the number of
antennas), whose entry $p$ is equal to $\Delta t_{p0}$. If $\bm{\Delta
  t_{pq}}$ is a vector of size $n_{\mathrm{bl}}$ (number of baselines) containing
the estimated $\widehat{\Delta t_{pq}}$ (Eq. \ref{eq:tpq}), and $\bm{\Pi}$ is a
matrix of size $n_{bl}\times n_a$, we can write our problem as a linear system:

\begin{alignat}{3}
\bm{\Delta t_{pq}}&=\bm{\Pi}\bm{\Delta t}\\
\text{with }\bm{\Pi}_{i,j}&=
 \begin{cases}
        1 \text{ if } j=p\\
        -1 \text{ if } j=q\\
        0 \text{ otherwise }
        \end{cases}
\end{alignat}

We then find the least square $\widehat{\bm{\Delta t}}$ solution using the
pseudo-inverse of $\bm{\Pi}$:

\begin{alignat}{3}
\widehat{\bm{\Delta t}}&=\left(
\bm{\Pi}^T\bm{\Pi}\right)^{-1}
\bm{\Pi}^T\bm{\Delta t_{pq}}
\end{alignat}


\subsection{Levenberg-Marquardt step}

In order to estimate $\widehat{\textbf{x}}_{0\mid
  0}$, we use a Levenberg-Marquardt least square minimization
algorithm, coupled with a Tikhonov-type regularization \citep[see for example][]{Eriksson96}. The algorithm 
computes a direction $\widehat{\Bdelta}$, and evolves $\widehat{\textbf{x}}_i$ following 
$\widehat{\textbf{x}}_{i+1}=\widehat{\textbf{x}}_{i}+\alpha\widehat{\Bdelta}$.

Starting by linearising
$\textbf{h}$ around $\widehat{\textbf{x}_i}$ we get
$\textbf{h}(\textbf{x})\approx\textbf{h}(\textbf{x}_i)+\MJx\Bdelta$ with $\Bdelta=\textbf{x}-\textbf{x}_i$. 
The $\chi^2$ can be written as:

\begin{alignat}{3}
\label{eq:Init_chi2}
&&\chi^2(\Bdelta)&=\| \MJx\Bdelta-\tilde{\textbf{z}}\|^2_\textbf{P} + \|\Bdelta+\textbf{x}_i-\textbf{x}_0\|^2_{\textbf{Q}^\gamma_0}\\
&&\text{with }\tilde{\textbf{z}}&=\textbf{z}-\textbf{h}(\textbf{x}_i)
\end{alignat}

\noindent As in Sec. \ref{sec:ImplAMM}
 $\|\textbf{x}\|_{\textbf{C}}=\textbf{x}^T\textbf{C}^{-1}\textbf{x}$,
is the norm of \textbf{x} for the metric
\textbf{C}. We minimize $\chi^2(\Bdelta)$ by solving:

\begin{alignat}{3}
\nonumber\frac{\partial \chi^2}{\partial \Bdelta}(\widehat{\Bdelta})&=0=&&\frac{1}{N}\MJx^T\textbf{P}^{-1}(\textbf{z}-\MJx\Bdelta)+\\
&&&\frac{1}{M}\textbf{Q}^{\gamma,-1}_0(\Bdelta+\textbf{x}_i-\textbf{x}_0)
\end{alignat}

\noindent and the direction of the minimum $\chi^2$ is:

\begin{alignat}{3}
\nonumber&\widehat{\Bdelta}&=&\frac{1}{N}\MJd\MJx\textbf{P}^{-1}(\textbf{z}-\textbf{h}(\textbf{x}_i))\\
&             &&+\frac{1}{M}\MJd\textbf{Q}^{\gamma,-1}_0(\textbf{x}_i-\textbf{x}_0)\\
\text{with }&\MJd&=&\left(\frac{1}{N}\MJx\textbf{P}^{-1}\MJx^T+\frac{1}{M}\textbf{Q}^{\gamma,-1}_0\right)^{-1}
\end{alignat}



%\section{Poststamps for }


==> ME_Simul_IonClock.tex <==

%%$\Delta t^d_{ion,pq}\propto \Delta\text{T}^d_{pq}/\nu^2$\\
%%$\Delta \phi^d_{ion,pq}=k. \Delta\text{T}^d_{pq}/\nu$

%% \begin{alignat}{3}
%% \textbf{V}^{meas}_{pq} &=& \textbf{G}_p\left(\displaystyle\sum\limits_{\vec{s}}\textbf{D}_{p,\vec{s}}\textbf{K}_{p,\vec{s}}\textbf{X}_{\vec{s}}\ 
%% \textbf{K}^H_{q,\vec{s}}\textbf{D}^H_{q,\vec{s}}\right)\textbf{G}^H_q \\ 
%% \end{alignat}

%$\textbf{D}^d_{p}:=\lambda^d_{ion}\textbf{I}$ and $\textbf{G}_p:=\lambda_{clock}\textbf{I}$

%% \begin{alignat}{3}
%% \textbf{D}^d_{p}&:=&&\exp(2\pi i \nu\ \delta t_{p0})\textbf{I}\\
%% %\nonumber\lambda_{clock} &=&& \\
%% \textbf{G}_p&:=&&\exp(i k\ \delta\text{T}^d_{p}/\nu)\textbf{I}\\
%% \delta t_{p0}&=&&\textbf{e}_{\textbf{clk}}(\textbf{x})\\
%% \delta\text{T}^d_{p}&=&&\textbf{e}_{\textbf{ion}}(\textbf{x})
%% %\nonumber\lambda^d_{ion} &=&& 
%% %\lambda_{clock}
%% \end{alignat}

%% \begin{alignat}{3}
%% \textbf{D}^d_{p}(\textbf{x})&:=&&\exp\left(i k\nu^{-1}\ \bm{\delta}\textbf{T}^\textbf{d}_{\textbf{p}}(\textbf{x}) \right)\textbf{I}\\
%% %\nonumber\lambda_{clock} &=&& \\
%% \textbf{G}_p(\textbf{x})&:=&&\exp\left(2\pi i \nu\ \bm{\delta}\textbf{t}_{\textbf{p0}}(\textbf{x})\right)\textbf{I}
%% %\delta t_{p0}&=&&\textbf{e}_{\textbf{clk}}(\textbf{x})
%% %\nonumber\lambda^d_{ion} &=&& 
%% %\lambda_{clock}
%% \end{alignat}

%% \begin{alignat}{5}
%% \textbf{D}^d_{p,t,\nu}(\textbf{x}):& \mathbb{R}^{N}\rightarrow \mathbb{R}^8\\
%% \nonumber          & \textbf{x}\mapsto \exp\left(i k\nu^{-1}\ \bm{\delta}\textbf{T}^d_{p,t}(\textbf{x}) \right)\textbf{I}\\
%% \textbf{G}_{p,t,\nu}(\textbf{x}):& \mathbb{R}^{N}\rightarrow \mathbb{R}^8\\
%% \nonumber          & \textbf{x}\mapsto \exp\left(2\pi i \nu\ \bm{\delta}\textbf{t}_{p,t}(\textbf{x})\right)\textbf{I}
%% \end{alignat}


\begin{alignat}{3}
%% \textbf{V}^{meas}_{pq}=\textbf{h}(\textbf{x}) &=&& \textbf{G}_p\left(\displaystyle\sum\limits_{d}\textbf{D}_{p,d}\textbf{K}_{p,d}\textbf{X}_{d}\ 
%% \textbf{K}^H_{q,d}\textbf{D}^H_{q,d}\right)\textbf{G}^H_q \\ 
%% \textbf{V}^{meas}_{pq}=\textbf{h}(\textbf{x}) &=&& \textbf{G}_p(\textbf{x})\left(\displaystyle\sum\limits_{d}\textbf{D}_{p,d}(\textbf{x})\textbf{K}_{p,d}\textbf{X}_{d}\ 
%% \textbf{K}^H_{q,d}\textbf{D}^H_{q,d}(\textbf{x})\right)\textbf{G}^H_q(\textbf{x}) \\ 
%% \textbf{V}^{meas}_{pq}=\textbf{h}(\textbf{x}) &=&& \textbf{G}_p(\textbf{x})\left(\displaystyle\sum\limits_{d}
%% \textbf{V}^{d}_{pq}(\textbf{x})
%% \right)\textbf{G}^H_q(\textbf{x}) \\ 
%% \textbf{V}^{d}_{pq}(\textbf{x})&=&& \textbf{D}_{p,d}(\textbf{x})\textbf{K}_{p,d}\textbf{X}_{d}\ \textbf{K}^H_{q,d}\textbf{D}^H_{q,d}(\textbf{x})\\
\textbf{D}^d_{p}(\textbf{x})&:=&&\exp\left(i k\nu^{-1}\ \bm{\delta}\textbf{T}^\textbf{d}_{\textbf{p}}(\textbf{x}) \right)\textbf{I}\\
%\nonumber\lambda_{clock} &=&& \\
\textbf{G}_p(\textbf{x})&:=&&\exp\left(2\pi i \nu\ \bm{\delta}\textbf{t}_{\textbf{p0}}(\textbf{x})\right)\textbf{I}
%\delta t_{p0}&=&&\textbf{e}_{\textbf{clk}}(\textbf{x})
%\nonumber\lambda^d_{ion} &=&& 
%\lambda_{clock}
\end{alignat}


==> MathKalman.tex <==


%%  Predict ===
%% $$\hat{\textbf{x}}_{k\mid k-1} = \textbf{F}_{k}\hat{\textbf{x}}_{k-1\mid k-1} + \textbf{B}_{k} \textbf{u}_{k-1}  $$
%% $$\textbf{P}_{k\mid k-1} =  \textbf{F}_{k} \textbf{P}_{k-1\mid k-1} \textbf{F}_{k}^{\text{T}} + \textbf{Q}_{k}$$

%% === Update ===
%% Innovation or measurement residual
%% $$\tilde{\textbf{y}}_k = \textbf{z}_k - \textbf{H}_k\hat{\textbf{x}}_{k\mid k-1}$$

%% Innovation (or residual) covariance
%% $$\textbf{S}_k = \textbf{H}_k \textbf{P}_{k\mid k-1} \textbf{H}_k^\text{T} + \textbf{R}_k $$

%% ''Optimal'' Kalman gain
%% $$\textbf{K}_k = \textbf{P}_{k\mid k-1}\textbf{H}_k^\text{T}\textbf{S}_k^{-1}$$

%% Updated (''a posteriori'') state estimate
%% $$\hat{\textbf{x}}_{k\mid k} = \hat{\textbf{x}}_{k\mid k-1} + \textbf{K}_k\tilde{\textbf{y}}_k$$

%% Updated (''a posteriori'') estimate covariance
%% $$\textbf{P}_{k|k} = (I - \textbf{K}_k \textbf{H}_k) \textbf{P}_{k|k-1}$$


Predict step



==> MathUKF.tex <==

%\def\mathbi#1{\textbf{\em #1}}


\begin{figure*}
\fbox{
  \parbox{\textwidth}{
As with the EKF, the UKF prediction can be used independently from the UKF update, in combination with a linear (or indeed EKF) update, or vice versa.
As with the EKF, the UKF prediction can be used independently from the UKF update, in combination with a linear (or indeed EKF) update, or vice versa.
As with the EKF, the UKF prediction can be used independently from the UKF update, in combination with a linear (or indeed EKF) update, or vice versa.
$\mathY$
  }
}
\caption{mes couilles}
\end{figure*}



Predict

As with the EKF, the UKF prediction can be used independently from the UKF update, in combination with a linear (or indeed EKF) update, or vice versa.

The estimated state and covariance are augmented with the mean and covariance of the process noise.

$$ \textbf{x}_{k-1\mid k-1}^{a} = [ \hat{\textbf{x}}_{k-1\mid k-1}^{T} \quad E[\textbf{w}_{k}^{T}] \ ]^{T} $$

%$$ \textbf{P}_{k-1\mid k-1}^{a} = \begin{bmatrix} & \textbf{P}_{k-1\mid k-1} & & 0 & \\ & 0 & &\textbf{Q}_{k} & \end{bmatrix} $$

A set of 2L+1 sigma points is derived from the augmented state and covariance where L is the dimension of the augmented state.


\begin{align}
\chi_{k-1\mid k-1}^{0} & = \textbf{x}_{k-1\mid k-1}^{a} \\[6pt]
\chi_{k-1\mid k-1}^{i} & =\textbf{x}_{k-1\mid k-1}^{a} + \left ( \sqrt{ (L + \lambda) \textbf{P}_{k-1\mid k-1}^{a} } \right )_{i}, \qquad i = 1,\ldots,L \\[6pt]
\chi_{k-1\mid k-1}^{i} & = \textbf{x}_{k-1\mid k-1}^{a} - \left ( \sqrt{ (L + \lambda) \textbf{P}_{k-1\mid k-1}^{a} } \right )_{i-L}, \qquad i = L+1,\dots{}2L
\end{align}


where

$$\left ( \sqrt{ (L + \lambda) \textbf{P}_{k-1\mid k-1}^{a} } \right )_{i}$$

is the ''i''th column of the matrix square root of

$$(L + \lambda) \textbf{P}_{k-1\mid k-1}^{a}$$

using the definition: square root ''A'' of matrix ''B'' satisfies

$$B \triangleq A A^T. \, $$

The matrix square root should be calculated using numerically efficient and stable methods such as the [[Cholesky decomposition]].

The sigma points are propagated through the transition function ''f''.

$$\chi_{k\mid k-1}^{i} = f(\chi_{k-1\mid k-1}^{i}) \quad i = 0,\dots,2L $$

where $$f : R^{L} \rightarrow R^{|\textbf{x}|} $$. The weighted sigma points are recombined to produce the predicted state and covariance.

$$\hat{\textbf{x}}_{k\mid k-1} = \sum_{i=0}^{2L} W_{s}^{i} \chi_{k\mid k-1}^{i} $$

$$\textbf{P}_{k\mid k-1} = \sum_{i=0}^{2L} W_{c}^{i}\ [\chi_{k\mid k-1}^{i} - \hat{\textbf{x}}_{k\mid k-1}] [\chi_{k\mid k-1}^{i} - \hat{\textbf{x}}_{k\mid k-1}]^{T} $$

where the weights for the state and covariance are given by:

$$W_{s}^{0} = \frac{\lambda}{L+\lambda}$$
$$W_{c}^{0} = \frac{\lambda}{L+\lambda} + (1 - \alpha^2 + \beta)$$
$$W_{s}^{i} = W_{c}^{i} = \frac{1}{2(L+\lambda)}$$
$$\lambda = \alpha^2 (L+\kappa) - L\,\! $$

$\alpha$ and $\kappa$ control the spread of the sigma points.  $\beta$ is related to the distribution of $x$.
Normal values are $\alpha=10^{-3}$, $\kappa=0$ and $\beta=2$. If the true distribution of $x$ is Gaussian, $\beta=2$ is optimal. 
%<ref>Wan, Eric A. and van der Merwe, Rudolph [http://www.lara.unb.br/~gaborges/disciplinas/efe/papers/wan2000.pdf "The Unscented Kalman Filter for Nonlinear Estimation"]</ref>

;Update

The predicted state and covariance are augmented as before, except now with the mean and covariance of the measurement noise.

$$ \textbf{x}_{k\mid k-1}^{a} = [ \hat{\textbf{x}}_{k\mid k-1}^{T} \quad E[\textbf{v}_{k}^{T}] \ ]^{T} $$

$$ \textbf{P}_{k\mid k-1}^{a} = \begin{bmatrix} & \textbf{P}_{k\mid k-1} & & 0 & \\ & 0 & &\textbf{R}_{k} & \end{bmatrix} $$

As before, a set of 2L+1 sigma points is derived from the augmented state and covariance where L is the dimension of the augmented state.


\begin{align}
\chi_{k\mid k-1}^{0} & = \textbf{x}_{k\mid k-1}^{a} \\[6pt]
\chi_{k\mid k-1}^{i} & = \textbf{x}_{k\mid k-1}^{a} + \left ( \sqrt{ (L + \lambda) \textbf{P}_{k\mid k-1}^{a} } \right )_{i}, \qquad i = 1,\dots,L \\[6pt]
\chi_{k\mid k-1}^{i} & = \textbf{x}_{k\mid k-1}^{a} - \left ( \sqrt{ (L + \lambda) \textbf{P}_{k\mid k-1}^{a} } \right )_{i-L}, \qquad i = L+1,\dots,2L
\end{align}


Alternatively if the UKF prediction has been used the sigma points themselves can be augmented along the following lines

$$ \chi_{k\mid k-1} := [ \chi_{k\mid k-1}^T \quad E[\textbf{v}_{k}^{T}] \ ]^{T} \pm \sqrt{ (L + \lambda) \textbf{R}_{k}^{a} }$$

where

$$ \textbf{R}_{k}^{a} = \begin{bmatrix} & 0 & & 0 & \\ & 0 & &\textbf{R}_{k} & \end{bmatrix} $$

The sigma points are projected through the observation function ''h''.

$$\gamma_{k}^{i} = h(\chi_{k\mid k-1}^{i}) \quad i = 0..2L $$

The weighted sigma points are recombined to produce the predicted measurement and predicted measurement covariance.

$$\hat{\textbf{z}}_{k} = \sum_{i=0}^{2L} W_{s}^{i} \gamma_{k}^{i} $$

$$\textbf{P}_{z_{k}z_{k}} = \sum_{i=0}^{2L} W_{c}^{i}\ [\gamma_{k}^{i} - \hat{\textbf{z}}_{k}] [\gamma_{k}^{i} - \hat{\textbf{z}}_{k}]^{T} $$

The state-measurement cross-covariance matrix,

$$\textbf{P}_{x_{k}z_{k}} = \sum_{i=0}^{2L} W_{c}^{i}\ [\chi_{k\mid k-1}^{i} - \hat{\textbf{x}}_{k\mid k-1}] [\gamma_{k}^{i} - \hat{\textbf{z}}_{k}]^{T} $$

is used to compute the UKF Kalman gain.

$$K_{k} = \textbf{P}_{x_{k}z_{k}} \textbf{P}_{z_{k}z_{k}}^{-1}$$

As with the Kalman filter, the updated state is the predicted state plus the innovation weighted by the Kalman gain,

$$\hat{\textbf{x}}_{k\mid k} = \hat{\textbf{x}}_{k\mid k-1} + K_{k}( \textbf{z}_{k} - \hat{\textbf{z}}_{k} )$$

And the updated covariance is the predicted covariance, minus the predicted measurement covariance, weighted by the Kalman gain.

$$\textbf{P}_{k\mid k} = \textbf{P}_{k\mid k-1} - K_{k} \textbf{P}_{z_{k}z_{k}} K_{k}^{T} $$


==> NoiseProps.tex <==
\section{Noise properties}
\label{sec:NoiseProps}

Applying any of the
representation operators presented above modifies the properties
of the input data covariance matrix $\MR$ (Eq. \ref{eq:KF_Sk},
\ref{eq:UKF_Pzzh}, and \ref{eq:UKF_Pzzh_S}). Assuming the
noise in the visibilities is uncorrelated, $\MR$ is diagonal
matrix. Assuming the noise is not baseline or frequency dependent we have
$\MR=\sigma^2\ \bm{\mathcal{I}}$, for $\RepUV$ and $\RepUVRe$,
and $\MR=(\sigma^2/n_\nu)\ \bm{\mathcal{I}}$ for $\RepImRe$. The
statistics of $\RepImAbs$ are non-Gaussian since it is the norm of a
complex number. The random variable is in that case $X=\sigma^{-1}\sqrt{n_\nu}\sqrt{
  (Re^2+Im^2)}$ which follows a non-central $\chi$-distribution with
2-degrees of freedom, and mean and covariance:

\begin{alignat}{3}
\mu_X&=\sqrt{\frac{\pi}{2}}L_{1/2}^{0}\left\{\frac{-\lambda^2}{2}\right\}\\
\sigma_X^2&=2+\lambda^2-\mu_X^2\\
\text{with }\lambda&=\sqrt{n_\nu}\sigma^{-1}\sqrt{\mu_{Re}^2+\mu_{Im}^2}
\end{alignat}

\noindent where $L_{1/2}^{0}$ is a generalized Laguerre polynomial.

